Adore: Differentially Oblivious Relational Database Operators

There has been a recent effort in applying differential privacy on memory access patterns to enhance data privacy. This is called differential obliviousness. Differential obliviousness is a promising direction because it provides a principled trade-off between performance and desired level of privacy. To date, it is still an open question whether differential obliviousness can speed up database processing with respect to full obliviousness. In this paper, we present the design and implementation of three new major database operators: selection with projection, grouping with aggregation, and foreign key join. We prove that they satisfy the notion of differential obliviousness. Our differentially oblivious operators have reduced cache complexity, runtime complexity, and output size compared to their state-of-the-art fully oblivious counterparts. We also demonstrate that our implementation of these differentially oblivious operators can outperform their state-of-the-art fully oblivious counterparts by up to $7.4\times$.

==> proofs.tex <==
\section{Differential Obliviousness Proofs}
\label{sec:proof}
\begin{theorem}[Main result for filter](restating Theorem \ref{thm:dofilter})
For any  $\epsilon \in (0,1)$, $\delta \in (0,1)$ and input $I$ with $N$ tuples , there is an ($\epsilon, \delta$)-differentially oblivious and distance preserving filtering algorithm ({\filteralg} in Algorithm~\ref{alg:dofilter}) that uses  $O(\log(1/\epsilon) \cdot \log^{1.5}N \cdot \log ( N/\delta))$
private memory and  $(N+R)/B$ cache complexity
\end{theorem}
\begin{proof}
First, we prove \autoref{alg:dofilter} is ($\epsilon, 0$)-differential oblivious if $P$ has infinite capacity:
For two neighboring input $I, I'$, assuming $I, I'$, we only leaks $\tilde{Y}_k$ 
($k=s, 2s, \ldots, n)$. This leakage is bounded by leaking 
all $\tilde{Y}_i$ ($i \in [N]$).
From the DP guarantee provided by the DP prefix sum oracle~\cite{css10}, all writes have at most ($\epsilon, 0$)-DP 
leakage.

Second, we prove \autoref{alg:dofilter} has at most $\delta$ 
probability of privacy failure with 
$O(\log(1/\epsilon) \cdot \log^{1.5} N \cdot \log (N/\delta) )$ private memory. 
Let $s = O(\log(1/\epsilon) \cdot \log^{1.5} N \cdot \log (N/\delta ))$.
We set $P = 2s$. 
Let $Y_c$ denote number of actual filtered tuples generated so far
(at line 14). From 
the DP guarantee provided by the DP prefix sum oracle, 
we know that for each $c$, 
$Y_c - s \leq \tilde{Y}_c \leq Y_c + s$ with $1 - \frac{\delta}{N}$ 
probability. By the union bound, we know that for all rounds of batched read, with at least 
$1 - \delta$ probability, $P$ over-flows or $P$ under-flows:
\begin{align*}
\Pr[Y_c-(\tilde{Y}_c - s) > 2s \lor Y_c < \tilde{Y}_c - s] \geq 1 -\delta    
\end{align*}
%
Now we can conclude that the failure probability of \autoref{alg:dofilter} is at most $\delta$.

In \autoref{alg:dofilter}, 
the amount of read is $N$, the amount of write
is $\tilde{Y}_N + s$, from the utility-privacy
bound from the DP oracle~\cite{css10}, it is 
$R + \poly \log (N)$. 
In addition, all the read and write in Algorithm~\ref{alg:dofilter} is batched, with the batch size $s$. Thus, the cache complexity of \autoref{alg:dofilter} is $(N+R)/B$ as long as $s \geq B$.
\end{proof}

\begin{theorem}[Main result for group, group via hashing](restating Theorem~\ref{thm:dogrouph})
For any  $\epsilon \in (0,1)$, $\delta \in (0,1)$ and input $I$ with size $N$ and $O(\eps^{-1}\log^2(1/\delta))$ private memory $M$, there is an ($\epsilon, \delta$)-differentially oblivious and distance preserving grouping algorithm ({\grouphalg} in Algorithm~\ref{alg:dogrouph}) that uses  $M$
private memory and has $N/B+11NR/9MB$ cache complexity.
\end{theorem}

\begin{proof}
The only information that \autoref{alg:dofilter} leaks is
$k$, the number of sequential scans of $I$.
This only leaks $\tilde{G}$ though, 
since $M$ is public. Moreover, $\tilde{G}$ is $(\eps, \delta/2)$-differentially private. 
Thus, \autoref{alg:dogrouph} is $(\eps, 0)$-differentially oblivious if we ignore the failure case.

Next, we prove that the failure probability of \autoref{alg:dogrouph} is at most $\delta$. 
Since $\sqrt{ 0.5 \tilde{G} \log (2k/\delta) } \leq 0.1M $ (line 4) and the expected number of group generated in each sequential scan is $0.9M$, let $G_i$
be the number of groups $i$-th sequential scan generated. From the properties of binomial distribution (detailed lemmas can be found in \autoref{sec:rand_partition}),
we have $\Pr[G_i \leq M] \leq \delta/2k$.
Applying a union bound over $k$ scans, we can bound the failure probability of the randomized partitioning by at most $\delta/2$. Applying union bound again with the $(\eps, \delta)$-differentially private $\tilde{G}$, we can bound the failure probability of \autoref{alg:dogrouph} to at most $\delta$.

Finally, \autoref{alg:dogrouph} requires a sequential scan of input in preprocessing, which takes $N/B$ I/O.
In the following steps, it requires $k(M + N) /B$ I/O, where $k \leq 1.1 R/ 0.9M$, which is no more than 
$\frac{11R(M+N)}{9MB}$. Here $M$ is absorbed by $N$. Thus, the overall cache complexity of \autoref{alg:dogrouph} is $N/B + 11NR/9MB$.

\end{proof}

\iffalse
\lianke{because we removed sort groupby, this part is comment out}
\begin{theorem}[Main result for group,  group via sorting](restating Theorem \ref{thm:dogroups})
For any  $\epsilon \in (0,1)$, $\delta \in (0,1)$ and input of size $N$, there is an ($\epsilon, \delta$)-differentially oblivious grouping algorithm ({\groupsalg} in Algorithm~\ref{alg:dogroups}) that uses  $O(\log(1/\epsilon) \cdot \log^{1.5}N \cdot \log ( 1/\delta))$
private memory and  $6 ( N / B ) \log_B (N/B) + (N+R)/B$ cache complexity. 
\end{theorem}
\begin{proof}
The proof of differential obliviousness follows the proof of \autoref{thm:dofilter}. Note that since \textsc{BucketOblivousSort} is fully oblivious, adding it as a preprocessing step does not change the differential obliviousness result.

The cache complexity of \textsc{BucketOblivousSort} is  $6 ( N / B ) \log (N/B)$. For the rest of the algorithm, the total read and write is $N+R$. And since both reads and writes are batched, as long as the batch size is greater than $B$, the cache complexity of the rest of the algorithm is $(N+R)/B$. Thus, we have demonstrated the cache complexity claim.
\end{proof}
\fi



\begin{theorem}[Main result for join](restating Theorem ~\ref{thm:dojoin})
For any  $\epsilon \in (0,1)$, $\delta \in (0,1)$, input $I$ with size $N$,
private memory of size $M$ and result size $R$, there is an ($\epsilon, \delta$)-differentially oblivious foreign key join algorithm (DoJoin in \autoref{alg:dojoin}) that uses  $O(\log(1/\epsilon) \cdot \log^{1.5}N \cdot \log ( N/\delta))$
private memory and has $6 (N/B) \log(N/B) + (N+R)/B$ cache complexity. 
\end{theorem}

\begin{proof}
\textsc{DoJoin} is $(\eps, \delta)$-differentially oblivious follows that \textsc{BucketObliviousSort} is fully oblivious and 
\textsc{DoFilter} is $(\eps, \delta)$-differentially oblivious
with $O(\log(1/\epsilon) \cdot \log^{1.5}N \cdot \log ( N/\delta))$ private memory. 

\textsc{DoJoin} requires sorting $R' || S'$ obliviously once. It uses \textsc{BucketOblivousSort}, which has cache complexity 
$6(N/B) \log{N/B}$. Additionally, the \textsc{DoFiler} algorithm it uses to get rid of filler tuples has cache complexity $(N+R)/B$. Thus, the cache complexity of \textsc{DoJoin} is $6 (N/B) \log(N/B) + (N+R)/B$
\end{proof}
